Analysis of a space-time unfitted finite element method for PDEs on evolving surfaces

In this paper we analyze a space-time unfitted finite element method for the discretization of scalar surface partial differential equations on evolving surfaces. For higher order approximations of the evolving surface we use the technique of (iso)parametric mappings for which a level set representation of the evolving surface is essential. We derive basic results in which certain geometric characteristics of the exact space-time surface are related to corresponding ones of the numerical surface approximation. These results are used in an error analysis of a higher order space-time TraceFEM.

==> deform_discontinuity.tex <==
\begin{figure}[!htbp]
	\centering
	\begin{tikzpicture}[scale = 2.3]
		\newdimen\XCoord
		\newdimen\YCoord
		\newcommand{\shgrid}{dotted}
		\newcommand{\ptsize}{0.7pt}
		\newcommand{\drawmesh}[4]{
			%horizontal lines of mesh
			\filldraw[#3, #4] (#1+0,#2+0) circle (\ptsize) -- (#1+1,#2+0) circle (\ptsize) -- (#1+2,#2+0) circle (\ptsize) -- (#1+3,#2+0) circle (\ptsize) ;
			\filldraw[#3, #4] (#1+0,#2+1) circle (\ptsize) -- (#1+1,#2+1) circle (\ptsize) -- (#1+2,#2+1) circle (\ptsize) -- (#1+3,#2+1) circle (\ptsize) ;
			\filldraw[#3, #4] (#1+0,#2+2) circle (\ptsize) -- (#1+1,#2+2) circle (\ptsize) -- (#1+2,#2+2) circle (\ptsize) -- (#1+3,#2+2) circle (\ptsize)  ;
			%vertical lines of mesh
			\filldraw[#3, #4] (#1+0,#2+0) -- (#1+0,#2+1) -- (#1+0,#2+2) ;
			\filldraw[#3, #4] (#1+1,#2+0) -- (#1+1,#2+1) -- (#1+1,#2+2);
			\filldraw[#3, #4] (#1+2,#2+0) -- (#1+2,#2+1) -- (#1+2,#2+2);
			\filldraw[#3, #4] (#1+3,#2+0) -- (#1+3,#2+1) -- (#1+3,#2+2) ;
		}
		
		%Mesh fillings
		
		\filldraw[red!70] (1,0) -- (1,1) -- (1,2) --  (3,2) --  (3,1) --  (2,1) -- (2,0);
		%Draw mesh
		\drawmesh{0}{0}{}{}
		%S_lin
		\draw[blue] (1,-0.3) .. controls (1.2, 0.3) .. (1.55,1);
		\draw[blue] (1.55,1) .. controls (1.7, 1.2) .. (2, 1.3);
		\draw[blue] (2,1.3) .. controls (2.52, 1.9) .. (2.9, 2.3);
		\node[scale=1, blue] at (2.6, 2.2) {$S_{\lin}$};
		%S_h
		\draw[blue!60!green] (1.1,-0.3) .. controls (1.2, 0.3) .. (1.92,1);
		\draw[blue!60!green] (1.7,1) .. controls (1.9, 1.1) .. (2, 1.2);
		\draw[blue!60!green] (2,1.2) .. controls (2.52, 1.7) .. (3, 2.3);
		\node[scale=1, blue!60!green] at (3.1, 2.2) {$S_h$};
		%Beschriftung Zeitschritte
		\node[scale=1] at (-0.3, 0) {$t_{n-1}$};
		\node[scale=1] at (-0.3, 1) {$t_{n}$};
		\node[scale=1] at (-0.3, 2) {$t_{n+1}$};
		%Beschriftung Omega_n etc
		\draw [decorate,decoration={brace,amplitude=3pt, mirror},xshift=0,yshift=-2pt]
		(1,0) -- (2,0) node [red,midway,yshift=-0.32cm] 
		{ $\Omega^\Gamma_{n}$};
		
		
		\draw [decorate,decoration={brace,amplitude=3pt},xshift=0,yshift=2pt]
		(1,2) -- (3,2) node [red,midway,yshift=0.32cm] 
		{ $\Omega^\Gamma_{n+1}$};
		
		
		%Beschriftung unstetigkeit
		\node[scale=1] at (1.28, 0.85) {$\Theta_{h}^{n}$};
		\draw[->, thick] (1.09,0.7) -- (1.09,0.99);
		\node[scale=1] at (1.37, 1.15) {$\Theta_{h}^{n+1}$};
		\draw[->, thick] (1.09,1.3) -- (1.09,1.01);
		%Beschriftung Qs
		\node[scale=1] at (3.35, 0.5) {$Q_{n}^{S}$};
		\node[scale=1] at (3.4, 1.5) {$Q_{n+1}^{S}$};
		\node[scale=1] at (1.6, 0.1) {$K_1$};
		\node[scale=1] at (2.6, 0.1) {$K_2$};
		\node[scale=1] at (2.1, 0.9) {$F$};
		
		
	\end{tikzpicture}
	\caption{Sketches of the discrete manifolds $S_{\lin}$ and $S_h$. Other than $S_{\lin}$, the surface $S_h$ is not necessarily continuous. In the calculation of ${\Theta_{h}^{n}(K_1\times I_n)}$ the degrees of freedom on the face $F$ only depend on $K_1$. In the calculation of ${\Theta_{h}^{n+1}(K_1\times I_{n+1})}$ the same degrees of freedoms depend on ${K_2\in\T^\Gamma_{n+1}}$ as well.}
	\label{deform_disc}
\end{figure}

